How Long Will My Phone Battery Last?

Mobile devices are only as useful as their battery lasts. Unfortunately, the operation and life of a mobile device's battery degrade over time and usage. The state-of-health (SoH) of batteries quantifies their degradation, but mobile devices are unable to support its accurate estimation -- despite its importance -- due mainly to their limited hardware and dynamic usage patterns, causing various problems such as unexpected device shutoffs or even fire/explosion. To remedy this lack of support, we design, implement and evaluate V-Health, a low-cost user-level SoH estimation service for mobile devices based only on their battery voltage, which is commonly available on all commodity mobile devices. V-Health also enables four novel use-cases that improve mobile users' experience from different perspectives. The design of V-Health is inspired by our empirical finding that the relaxing voltages of a device battery fingerprint its SoH, and is steered by extensive measurements with 15 batteries used for various commodity mobile devices, such as Nexus 6P, Galaxy S3, iPhone 6 Plus, etc. These measurements consist of 13,377 battery discharging/charging/resting cycles and have been conducted over 72 months cumulatively. V-Health has been evaluated via both laboratory experiments and field tests over 4-6 months, showing <5% error in SoH estimation.

==> discussion.tex <==


\section{Discussion: Extending Dataset}
\label{sec:discussion}

Ideally, \nameS is to be provided by OEMs because of their accessibility to battery cycling datasets, 
e.g., covering a complete battery SoH range.
%
In case a limited dataset is available, it can be extrapolated based on the linearity between voltage drop 
during resting and battery SoH~\cite{H}. 
%
Again, we used the cycling measurements in Fig.~\ref{fig:VoltageandSoH} to show this observation.
%
Fig.~\ref{fig:extendingdataset} plots the voltage drop after the battery is rested for $10$, $20$ and $30$ minutes  
during the resting period of each cycle, together with the corresponding battery SoH during that cycle. 
We can see clear linearity in all three traces of dropped voltage, with RMSE in the order of $10^{-4}$.
%
This observation enables us to identify the linear coefficients based on the available cycling dataset, 
generate relaxing voltages that correspond to uncovered SoH, and eventually construct the complete 
voltage fingerprint map. 










